Fine-grained Text and Image Guided Point Cloud Completion with CLIP Model

This paper focuses on the recently popular task of point cloud completion guided by multimodal information. Although existing methods have achieved excellent performance by fusing auxiliary images, there are still some deficiencies, including the poor generalization ability of the model and insufficient fine-grained semantic information for extracted features. In this work, we propose a novel multimodal fusion network for point cloud completion, which can simultaneously fuse visual and textual information to predict the semantic and geometric characteristics of incomplete shapes effectively. Specifically, to overcome the lack of prior information caused by the small-scale dataset, we employ a pre-trained vision-language model that is trained with a large amount of image-text pairs. Therefore, the textual and visual encoders of this large-scale model have stronger generalization ability. Then, we propose a multi-stage feature fusion strategy to fuse the textual and visual features into the backbone network progressively. Meanwhile, to further explore the effectiveness of fine-grained text descriptions for point cloud completion, we also build a text corpus with fine-grained descriptions, which can provide richer geometric details for 3D shapes. The rich text descriptions can be used for training and evaluating our network. Extensive quantitative and qualitative experiments demonstrate the superior performance of our method compared to state-of-the-art point cloud completion networks.

==> Feature_Visualization.tex <==
\subsection{Feature Visualization}
\begin{figure*}[h] 
  \centering
  \includegraphics[width=0.9\textwidth]{fig/moreviscomp.pdf}
  \caption{Comparisons between CSDN and its competitors~\cite{yu2021pointr,zhang2021view} when images and partial point clouds are captured under the same viewpoints.}
  \label{fig:morevis}
\end{figure*}

To better understand the role of IPAdaIN, this section provides visualizations of the features before and after IPAdaIN in the Shape Fusion module in two different ways. Specifically, we define the point-wise features before the last layer of IPAdaIN as $F_{before}=\{f_1,...,f_N\}\subseteq\mathbb{R}^C$, the corresponding point-wise features after IPAdaIN as $F_{after}$, and the generated coarse points as $P_{coarse}=\{p_1,...,p_N\}\subseteq\mathbb{R}^3$. Note that the affine transformation in IPAdaIN is the only step where image features are involved for point generation in the Shape Fusion module.

We first explore how features change before and after IPAdaIN. During the folding operation, points that are close in the 3D space should also be close in the feature space (i.e., $f_a$ should have a relatively small Euclidean distance to $f_b$ if $p_a$ and $p_b$ are spatially close). Figure~\ref{fig:feaeuvis} visualizes the coarse shapes $P_{coarse}$ generated by the Shape Fusion module, and the target points were randomly selected in the originally missing parts. Then, we compute the Euclidean distances between the target point and other points in the feature space. The visualization is generated by coloring points based on the distances. As shown in Figure~\ref{fig:feaeuvis}, points similar to the target point in the feature space are spread across the entire point cloud before IPadaIN. After IPadaIN, the similar points in the feature space become closer in the 3D space. It should be noted that IPAdaIN does not involve any learnable parameters other than the affine parameters generated by the image features. This means that the affine transformation of IPAdaIN changes the feature distributions and normalizes the generated points to the complete shape.

In addition, we plot $F_{before}$, $F_{after}$, and $P_{coarse}$ as 2D images by t-SNE~\cite{van2008visualizing} in Figure \ref{fig:feavis} to disclose the change in feature distribution after IPAdaIN. It can be concluded that IPAdaIN makes the distribution of point-wise feature $F_{after}$ more similar to its direct result $P_{coarse}$ than $F_{before}$. These results further explain that IPAdaIN fuses modalities by changing feature statistics.



==> README <==

December 27, 2012


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

V1.8 is a significant update over the 1.7a release. For a full list of
changes, please read the file changelog.txt. The most notable changes
include:


 1) New transmag class option to support the IEEE Transactions on Magnetics
    format. Thanks to Wei Yingkang, Sangmin Suh and Benjamin Gaussens
    for suggestions and beta testing.

 2) The \IEEEcompsoctitleabstractindextext and 
    \IEEEdisplaynotcompsoctitleabstractindextext
    commands have been deprecated in favor of their
    \IEEEtitleabstractindextext and \IEEEdisplaynontitleabstractindextext
    (observe that the "not" has changed to "non") equivalents. This change
    generalizes and decouples them from compsoc mode because the new
    transmag mode also uses them now.

 3) Added new *-forms of \IEEEyesnumber*, \IEEEnonumber*, \IEEEyessubnumber*,
    and \IEEEnosubnumber* (the non-star form of the latter is also new) which
    persist across IEEEeqnarray lines until countermanded. To provide for
    continued subequations across instances of IEEEeqnarrays as well as for
    subequations that follow a main equation (e.g., 14, 14a, 14b ...)
    \IEEEyessubnumber no longer automatically increments the equation number
    on it's first invocation of a subequation group. Invoke both
    \IEEEyesnumber\IEEEyessubnumber together to start a new
    equation/subequation group.
 
 4) Hyperref links now work with IEEEeqnarray equations.
    Thanks to Stefan M. Moser for reporting this problem.

 5) Revised spacing at top of top figures and tables to better
    align with the top main text lines as IEEE does in its journals. 
    Thanks to Dirk Beyer for reporting this issue and beta testing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> limitation.tex <==
\section{Limitations and Failure Cases}
Table~\ref{tab:limitations} summarizes the limitations among these compared methods to provoke further research insights. Besides, we visualize some failure cases whose CD losses are rather larger than the average error of that category, as shown in Figure \ref{fig:failure}. Although the shape fusion step succeeds in recovering the complete shape to a certain extent, and the dual-refinement module also removes noisy points, the final results are still less pleasing. This is especially the case when the partial point clouds have large missing regions both in their main bodies and detailed structures. Meanwhile, the input images are of very low resolutions, which can only provide limited complementary information for the recovery of fine geometries (e.g., the ship cabin). This problem could be solved by training on a dataset that has real-world high-resolution images and dense point clouds. Besides, although the motivation of the proposed CSDN is to reconstruct better shapes with the help of single-view images, multi-view images and neural rendering techniques would also help point cloud completion, which is our future work.

